OVO-Bench: How Far is Your Video-LLMs from Real-World Online Video Understanding?

Temporal Awareness, the ability to reason dynamically based on the timestamp when a question is raised, is the key distinction between offline and online video LLMs. Unlike offline models, which rely on complete videos for static, post hoc analysis, online models process video streams incrementally and dynamically adapt their responses based on the timestamp at which the question is posed. Despite its significance, temporal awareness has not been adequately evaluated in existing benchmarks. To fill this gap, we present OVO-Bench (Online-VideO-Benchmark), a novel video benchmark that emphasizes the importance of timestamps for advanced online video understanding capability benchmarking. OVO-Bench evaluates the ability of video LLMs to reason and respond to events occurring at specific timestamps under three distinct scenarios: (1) Backward tracing: trace back to past events to answer the question. (2) Real-time understanding: understand and respond to events as they unfold at the current timestamp. (3) Forward active responding: delay the response until sufficient future information becomes available to answer the question accurately. OVO-Bench comprises 12 tasks, featuring 644 unique videos and approximately human-curated 2,800 fine-grained meta-annotations with precise timestamps. We combine automated generation pipelines with human curation. With these high-quality samples, we further developed an evaluation pipeline to systematically query video LLMs along the video timeline. Evaluations of nine Video-LLMs reveal that, despite advancements on traditional benchmarks, current models struggle with online video understanding, showing a significant gap compared to human agents. We hope OVO-Bench will drive progress in video LLMs and inspire future research in online video reasoning. Our benchmark and code can be accessed at https://github.com/JoeLeelyf/OVO-Bench.

==> sec/tables/all_results.tex <==
% \begin{table}[h]
%     \centering
%     \begin{tabular}{lccccccc}
%         \toprule
%         \textbf{Model} & \textbf{CP} & \textbf{FP} & \textbf{IR} & \textbf{LR} & \textbf{ST} & \textbf{MA} & \textbf{Avg.} \\
%         \midrule
%         \multicolumn{8}{c}{\textit{Baselines}} \\
%         \midrule
%         Random Choice & 23.7 & 24.5 & 25.3 & 24.3 & 24.8 & 25.1 & 24.6 \\
%         \midrule
%         \multicolumn{8}{c}{\textit{Closed-source LLMs}} \\
%         \midrule
%         GPT4-Turbo\cite{34} & 2.4 & 4.0 & 9.6 & 18.0 & 13.6 & 25.6 & 12.2 \\
%         Gemini-Pro\cite{41} & \textbf{16.8} & \textbf{13.6} & \textbf{20.4} & \textbf{24.4} & \textbf{19.6} & \textbf{28.8} & \textbf{20.6} \\
%         \midrule
%         \multicolumn{8}{c}{\textit{Open-source LLMs}} \\
%         \midrule
%         Qwen1.5-1.8B\cite{1} & 28.4 & 28.4 & 25.6 & 23.2 & \textbf{23.2} & 29.6 & 26.4 \\
%         Phi2-2.7B\cite{32} & 11.2 & 11.2 & 15.2 & 10.8 & 11.6 & 12.0 & 12.0 \\
%         Yi-6B-Chat\cite{49} & 23.6 & 19.2 & 28.4 & 25.2 & 12.4 & 29.6 & 23.1 \\
%         LLaMA2-7B\cite{43} & 28.0 & \textbf{30.4} & 26.0 & 18.0 & 18.8 & 21.6 & 23.8 \\
%         Qwen-7B\cite{1} & 11.6 & 5.6 & 12.8 & 5.6 & 7.2 & 0.4 & 7.2 \\
%         Deepseek-7B\cite{3} & 26.8 & 16.0 & 28.4 & 21.6 & \textbf{23.2} & 25.6 & 23.6 \\
%         InternLM2-7B\cite{42} & 22.0 & 14.8 & 22.0 & 21.6 & 15.2 & 23.2 & 19.8 \\
%         Qwen1.5-7B\cite{1} & 15.6 & 8.0 & 9.2 & 9.2 & 15.2 & 9.2 & 11.1 \\
%         Vicuna-v1.5-7B\cite{8} & 22.0 & 27.6 & 29.6 & 26.4 & 18.0 & 24.4 & 24.7 \\
%         Baichuan2-7B\cite{47} & 20.8 & 18.4 & 27.6 & 18.8 & 18.8 & 21.2 & 20.9 \\
%         Mistral-7B\cite{18} & 20.0 & 23.6 & 24.4 & 23.6 & 20.0 & 27.2 & 23.1 \\
%         LLaMA2-13B\cite{43} & 23.6 & 23.6 & 28.0 & 21.2 & 16.4 & 10.4 & 20.5 \\
%         Vicuna-v1.5-13B\cite{8} & \textbf{32.8} & 24.0 & \textbf{28.8} & 17.6 & 22.0 & 14.4 & 23.3 \\
%         Baichuan2-13B\cite{47} & 26.4 & 18.0 & 28.0 & 20.4 & 21.2 & 25.6 & 23.3 \\
%         InternLM2-20B\cite{42} & 18.2 & 17.8 & 22.6 & 23.8 & 17.8 & 13.4 & 18.9 \\
%         Yi-34B\cite{49} & 20.4 & 18.0 & 24.0 & 24.0 & 14.4 & \textbf{30.8} & 21.9 \\
%         Mixtral-8x7B\cite{19} & 24.4 & 17.6 & 19.2 & \textbf{28.0} & 16.0 & 33.6 & 23.1 \\
%         Deepseek-67B\cite{3} & 29.2 & 22.4 & 18.4 & 26.0 & 20.4 & 22.4 & 23.1 \\
%         LLaMA2-70B\cite{43} & 22.4 & 20.0 & 19.6 & 14.4 & 7.2 & 9.6 & 15.5 \\
%         Qwen1.5-72B\cite{1} & 21.6 & 16.0 & 21.2 & 14.0 & 17.2 & 27.2 & 19.5 \\
%         \bottomrule
%     \end{tabular}
%     \caption{Performance comparison of various models across different tasks.}
%     \label{tab:performance}
% \end{table}

==> sec/tables/license.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{c|l}
        \toprule
        \textbf{Dataset} & \textbf{License}  \\
        \midrule
        Perception Test \cite{patraucean2024perception} & CC BY 4.0  \\
        Charades-STA \cite{gao2017tall,sigurdsson2016hollywood} & Non-Commercial Use  \\
        STAR \cite{wu2024star} & Apache License 2.0  \\
        QVHighlights \cite{lei2021qvhighlights} & CC BY-NC-SA 4.0  \\
        Ego4D-NLQ \cite{grauman2022ego4d} & Custom  \\
        THUMOS'14 \cite{jiang2014thumos} & Research Purpose Only \\
        THUMOS'15 \cite{gorban2015thumos} & Research Purpose Only  \\
        TVSum \cite{song2015tvsum} & CC BY 4.0  \\
        SumMe \cite{gygli2014creating} & N/A   \\
        YouTube Highlights \cite{sun2014ranking} & N/A   \\
        HiREST \cite{zala2023hierarchical} & MIT License  \\
        YouCook2 \cite{zhou2018towards} & MIT License  \\
        CrossTask \cite{zhukov2019cross} & BSD 3-Clause License  \\
        HT-Step \cite{afouras2024ht} & CC BY-NC 4.0  \\
        QAEgo4D \cite{barmann2022did} & N/A  \\
        \bottomrule
    \end{tabular}
\end{table}

==> sec/tables/task_dimensions.tex <==
\begin{table*}[t]
    \vspace{-2mm}
    \centering
    \vspace{1mm}
    \renewcommand{\arraystretch}{1.2}  % 增加行间距
    \resizebox{1.0\textwidth}{!}{%
% \begin{table}[tp]
% \centerings
% \resizebox{\textwidth}{!}{ % 使用\resizebox调整表格大小
\begin{tabular}{lcccccccccccll}
\hline
\multicolumn{1}{c|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{7}{c|}{\textbf{Real-Time Visual Perception}} &
  \multicolumn{4}{c|}{\textbf{Backward Tracing}} &
  \multicolumn{1}{c}{} \\ \cline{3-13}
\multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{Model}}} &
  \multicolumn{1}{l|}{\multirow{-2}{*}{\textbf{\# Frames}}} &
  OCR &
  ACR &
  ATR &
  STU &
  FTP &
  \multicolumn{1}{c|}{OJR} &
  \multicolumn{1}{c|}{Avg.} &
  EPM &
  ASI &
  \multicolumn{1}{c|}{HLD} &
  \multicolumn{1}{c|}{Avg.} &
  \multicolumn{1}{c}{\multirow{-2}{*}{\textbf{Overall}}} \\ \hline
\multicolumn{14}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Human}} \\ \hline
\multicolumn{1}{l|}{Human Agents} &
  \multicolumn{1}{c|}{-} &
  93.96 &
  92.57 &
  96.94 &
  93.33 &
  91.09 &
  \multicolumn{1}{c|}{97.48} &
  \multicolumn{1}{c|}{94.23} &
  - &
  - &
  \multicolumn{1}{c|}{-} &
  \multicolumn{1}{c|}{} &
   \\ \hline
\multicolumn{14}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Blind LLMs}} \\ \hline
\multicolumn{1}{l|}{GPT-4-turbo} &
  \multicolumn{1}{c|}{64} &
  28.86 &
  24.77 &
  27.55 &
  32.59 &
  27.72 &
  \multicolumn{1}{c|}{28.86} &
  \multicolumn{1}{c|}{28.39} &
  - &
  - &
  \multicolumn{1}{c|}{-} &
  \multicolumn{1}{c|}{} &
   \\ \hline
\multicolumn{14}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Proprietary Multimodal Models-Offline}} \\ \hline
\multicolumn{1}{l|}{GPT-4o} &
  \multicolumn{1}{c|}{64} &
  73.15 &
  \textbf{68.81} &
  77.55 &
  56.30 &
  \textbf{77.23} &
  \multicolumn{1}{c|}{62.42} &
  \multicolumn{1}{c|}{69.24} &
  55.22 &
  \textbf{76.74} &
  \multicolumn{1}{c|}{34.21} &
  \multicolumn{1}{c|}{} &
   \\
\multicolumn{1}{l|}{Gemini 1.5 Pro} &
  \multicolumn{1}{c|}{1fps} &
  \textbf{87.23} &
  65.12 &
  \textbf{82.65} &
  \textbf{61.48} &
  68.32 &
  \multicolumn{1}{c|}{\textbf{68.46}} &
  \multicolumn{1}{c|}{\textbf{72.21}} &
   &
  69.77 &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
   \\ \hline
\multicolumn{14}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Open-source Multimodal Models-Offline}} \\ \hline
\multicolumn{1}{l|}{Qwen2-VL-72B} &
  \multicolumn{1}{c|}{64} &
  \textbf{77.18} &
  \textbf{61.47} &
  \textbf{82.65} &
  53.33 &
  \textbf{76.24} &
  \multicolumn{1}{c|}{67.79} &
  \multicolumn{1}{c|}{\textbf{69.78}} &
  52.19 &
  69.77 &
  \multicolumn{1}{c|}{\textbf{63.16}} &
  \multicolumn{1}{l|}{} &
   \\
\multicolumn{1}{l|}{LLaVA-NeXT-Video-7B} &
  \multicolumn{1}{c|}{64} &
  74.50 &
  60.55 &
  68.37 &
  54.07 &
  72.28 &
  \multicolumn{1}{c|}{\textbf{68.46}} &
  \multicolumn{1}{c|}{66.37} &
  55.89 &
  76.74 &
  \multicolumn{1}{c|}{5.26} &
  \multicolumn{1}{l|}{} &
   \\
\multicolumn{1}{l|}{LLaVA-OneVision-7B} &
  \multicolumn{1}{c|}{64} &
  70.74 &
  59.63 &
  76.53 &
  50.37 &
  71.29 &
  \multicolumn{1}{c|}{67.79} &
  \multicolumn{1}{c|}{66.06} &
  \textbf{56.23} &
  76.74 &
  \multicolumn{1}{c|}{14.91} &
  \multicolumn{1}{l|}{} &
   \\
\multicolumn{1}{l|}{InternVL-V2-8B} &
  \multicolumn{1}{c|}{64} &
  73.15 &
  58.72 &
  70.14 &
  \textbf{57.04} &
  70.30 &
  \multicolumn{1}{c|}{63.76} &
  \multicolumn{1}{c|}{65.52} &
  48.48 &
  76.74 &
  \multicolumn{1}{c|}{28.95} &
  \multicolumn{1}{l|}{} &
   \\
\multicolumn{1}{l|}{Qwen2-VL-7B} &
  \multicolumn{1}{c|}{64} &
  70.74 &
  52.29 &
  69.39 &
  42.22 &
  71.29 &
  \multicolumn{1}{c|}{65.10} &
  \multicolumn{1}{c|}{61.84} &
  47.14 &
  76.74 &
  \multicolumn{1}{c|}{41.23} &
  \multicolumn{1}{l|}{} &
   \\
\multicolumn{1}{l|}{LongVU-7B} &
  \multicolumn{1}{c|}{1fps} &
  55.70 &
  54.13 &
  64.29 &
  40.74 &
  68.32 &
  \multicolumn{1}{c|}{61.74} &
  \multicolumn{1}{c|}{57.487} &
  50.17 &
  \textbf{81.40} &
  \multicolumn{1}{c|}{5.26} &
  \multicolumn{1}{l|}{} &
   \\ \hline
\multicolumn{14}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Open-source Multimodal Models-Online}} \\ \hline
\multicolumn{1}{l|}{Flash-VStream-7B} &
  \multicolumn{1}{c|}{1fps} &
  40.94 &
  51.38 &
  44.90 &
  38.52 &
  62.38 &
  \multicolumn{1}{c|}{44.97} &
  \multicolumn{1}{c|}{47.18} &
  \multicolumn{1}{l}{42.76} &
  \multicolumn{1}{l}{39.53} &
  \multicolumn{1}{l|}{4.39} &
  \multicolumn{1}{l|}{} &
   \\
\multicolumn{1}{l|}{VideoLLM-online-8B} &
  \multicolumn{1}{c|}{1fps} &
   &
   &
   &
   &
   &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
   \\ \hline
\end{tabular}
}
    \caption{Evaluation results on VideoCoTBench. \textdagger\ refers to using \textit{"low"} resolution.}
% 添加表格标题
\end{table*}
